Rule Enforcing Through Ordering

In many real world situations, like minor traffic offenses in big cities, a central authority is tasked with periodic administering punishments to a large number of individuals. Common practice is to give each individual a chance to suffer a smaller fine and be guaranteed to avoid the legal process with probable considerably larger punishment. However, thanks to the large number of offenders and a limited capacity of the central authority, the individual risk is typically small and a rational individual will not choose to pay the fine. Here we show that if the central authority processes the offenders in a publicly known order, it properly incentives the offenders to pay the fine. We show analytically and on realistic experiments that our mechanism promotes non-cooperation and incentives individuals to pay. Moreover, the same holds for an arbitrary coalition. We quantify the expected total payment the central authority receives, and show it increases considerably.

==> sections/analytic.tex <==
\section{Analytic Solution}
\label{sec: analytic}
While existence of an analytic solution of \gamename remains an open question, we can still find it in certain special cases. 
%Here, behavior of agents at the start of \agentset will prove crucial. This is because, if agents position is $n_a \le k$, he will pay $Q$ unless his payment $\mu_a$ is high enough to be sorted after at least $k$ other agents. 

\subsection{Active participants}
\label{ssec: p=0}
Let us first focus on a situation when no agent forgets to participate in \roundname, i.e. $p=0$.
Then it is easy to see that $\pi_a = \sigma^F$ is the only equilibrium. Indeed, if any agent chooses to deviate and pay $\mu_a< F$ instead then he is forced to pay $Q$ resulting in $u_a = -Q-\mu_a < F$.

\todo[inline]{D: See analytic_david for a better version}

\subsection{Charity-less system}
Let us focus on the system without the introduction of the charity. Then the agents are unable to make partial donations, and thus after scaling such that $F=1$.
When $F=1$, then agents can either pay nothing and risk paying $Q$, or pay the fine $F$ in each round.

\begin{definition}
\label{def.xxx}
Let $n$ be a positive integer. We denote by $\alpha(p,n,k)$ the probability that in $n-1$ independent coin tosses of the coin where the probability of the head is $p$, the number of heads is less than $k$.
\end{definition}

%\subsection{Bounds on $\alpha$}
%\label{sub.bal}
\begin{lemma}
\label{l.al}
For $k<np$, $$\alpha(p,n+1,k) \leq  e^{-\frac{\left( np-k \right)^2}{2np}}$$.
\end{lemma}
\begin{proof}
Let $X_i$ denote the random variable such that $$ X_i = \begin{cases}
  1  &  \text{ with probability } p, \\
  0 &   \text{ with probability } 1-p,
\end{cases}
$$
and $X^n = \underset{i=1}{\overset{n}{\sum}}X_i$. Thus, $\mathbb{E}[X_i]=p$ and $\mathbb{E}[X^n]=np$.
As per the Chernoff bounds, $\mathbb{P}[X^n \leq (1-\delta)np]\leq e^{\frac{-\delta^2np}{2}}$, for all $ 0<\delta<1$.
Thus $\alpha(p,n+1,K)=\mathbb{P}[X^n \leq k] \leq e^{{-\left( 1-\frac{k}{np} \right) ^2np}\slash{2}} = e^{-\frac{\left( np-k \right)^2}{2np}}$.

%When $np < K$. We can use Hoeffding inequality $\mathbb{P}[X^n - np \geq \delta]\leq e^{-\frac{-2\delta^2}{n}}$, $\forall$ $ 0<\delta$.

%Thus,
%\begin{align*}
%     \alpha(p,n+1,K) & = & 1-\mathbb{P}[X^n \geq K] \\ 
%     & = & 1-\mathbb{P}[X^n -np \geq K -np] \\
%     &\geq & 1- e^{-{2\left( \frac{K}{np} - 1 \right) ^2}\slash{n}} \\
%\end{align*}
%For $np<K<n$ we have,
%\begin{align*}
%     \alpha(p,n+1,K) & = & 1-\mathbb{P}[X^n \geq K] \\ 
%     &\geq & 1- e^{-n\left({\frac{K}{np}\log\left( \frac{K}{np} \right)} + \left(1 - \frac{K}{n} %\end{align*}

\end{proof}

%For the case of $np<k<n$, we refer to Theorem 1 of~\cite{Arratia1989TutorialOL}.
%\begin{theorem}[\cite{Arratia1989TutorialOL}]
%For $p<a<1$, $\mathbb{P}[X^n \geq an]\leq e^{-nH}$, where $H\equiv H(a,p)=a\log\left(\frac{a}{p}\right)+\left(1-a\right)\log\left(\frac{1-a}{1-p}\right)$
%\end{theorem}
%Setting $a=\frac{k}{n}$ and using $\alpha(p,n+1,k)  =  1-\mathbb{P}[X^n \geq k]$  we get the following bound.
%\begin{corollary}
%For $np<k<n$, $$\alpha(p,n+1,k) \geq 1- e^{-n\left({\frac{k}{np}\log\left( \frac{k}{np} \right)} + \left(1 - \frac{k}{n} \right)\log\left( \frac{1-\frac{k}{n}}{1-p} \right)\right)}$$
%\end{corollary}


%\begin{remark}
%Note that $H\geq0$ for all values of $a$ and $p$, moreover $H=0$ if and only if $a=p$. Thus as long as $np<k$, the bound on $\alpha(p,n+1,k)$ remains positive.
%\end{remark}
%\begin{remark}
%The case for $n<k$ is trivial as $\alpha(p,n+1,k)=1$.
%\end{remark}
%\begin{proof}
%We refer to Theorem 1 of~\cite{Arratia1989TutorialOL}. Which 
%\begin{align*}
%     \alpha(p,n+1,K) & = & 1-\mathbb{P}[X^n \geq K] \\ 
%     &\geq & 1- e^{-n\left({\frac{K}{np}\log\left( \frac{K}{np} \right)} + \left(1 - \frac{K}{n} \right)\log\left( \frac{1-\frac{K}{n}}{1-p} \right)\right)} \\
%\end{align*}
%\end{proof}



\begin{proposition}
\label{p.aa}
If $\alpha(p,n,k)\leq F/Q\leq \frac{1}{4}$ then $np > k$. Moreover for large enough $n$, $\alpha(p,n,k)\geq \alpha(p,2n,2k)$.
\end{proposition}
\begin{proof}

According to~\cite{GREENBERG201491} for $X\todo{D: X is already taken}\sim B(n,p)$, when $ p<1-\frac{1}{n}$, $\frac{1}{4}<\mathbb{P}[X\leq np]$. These bounds are tight. So when $\frac{1}{4}\geq \frac{F}{Q}$, we have $k<np$.

Further, we note that Lemma \ref{l.al} is tight for large enough $np$. Hence, it suffices to prove the proposition for the upper bound 
$$e^{-\frac{\left( np-k \right)^2}{2np}}$$
for which the statement clearly holds.

\end{proof}


\subsection{Gangster game}
\label{sub.g}

We start by analysing the charity-less system lasting only one step.
The \gamename with parameters $F=T=w=1$, $Q>F$ is called the {\em Gangster game}. It models a dramatic situation when there is a collection of shops which did not pay the protection money to a gang. The gang arranges the shops into a sequence and declares that first $k$ shops in the sequence which do not pay for the protection within one day will be burned.

Each {\em mixed strategy}\todo{D: This will not be a mixed strategy. The strategy is defined without ignorance, the environment makes you forget.} of the Gangster game thus assigns to each player $a$ a probability $p(a)\leq (1-p)$\todo{D: How does p depend on the agent? By definition of the Round, the strategy of $a$ is without ignorance. What does this mean?} to pay $F$.



\begin{definition}
\label{def.crit}
The smallest $r_1$ such that $\alpha(p,r_1,k)Q\leq F$ will be called {\em critical position}.

The mixed strategy ${\mathcal R}_1$ for a player $a$ of the Gangster game is: pay $F$ with probability $1-p$ if $\alpha(p,n_a,k)Q> F$ and pay $0$ otherwise\todo{D: The strategy is just to pay F or 0. Env makes you forget.}. 
\end{definition}





We prove that ${\mathcal R}_1$ is the only mixed equilibrium of the Gangster game, after establishing first the expected payoff, denoted by $G_1(p,n_a,k)$, of player $a$ assuming all players follow ${\mathcal R}_1$.

\begin{definition}
\label{def.expp}
We define the decisive function $c_1(p,n,k)$ of the strategy ${\mathcal R}_1$ and probability $\alpha'(p,n,k)$ as follows:
(1) If $n< r_1$ then $c_1(p,n,k)= \alpha(p,n,k)Q$ and $\alpha'(p,n,k)= \alpha(p,n,k)$, (2) If $n= r_1+i, 0\leq i\leq k-1$ then $c_1(p,n,k)= \alpha(p,r_1,k-i)Q$ and $\alpha'(p,n,k)= \alpha(p,r_1,k-i)$, and (3) $c_1(p,n,k)= \alpha'(p,n,k)= 0$ when $n\geq r_1+k$.
 \end{definition}

\begin{theorem}
\label{thm.p}
Let $r_1$ be the critical position and let all players follow ${\mathcal R}_1$. The expected payoff $G_1(p,n_a,k)$ of player $a$ is: (1) If $n_a< r_1$ then $G_1(p,n_a,k)= (1-p)F+ pc_1(p,n_a,k)$, (2) If $n_a\geq r_1$ then $G_1(p,n_a,k)= c_1(p,n_a,k)$. The total expected payoff, denoted by $T_1(p,x_0,k)$, is
$$
T_1(p,x_0,k)= -F(1-p)(r_1-1)- Qk.
$$\todo{D: Shouldn't there be $r_1$, not $(r_1- 1)$? Agent at $r_1$ will try to pay no?}
\end{theorem}


\begin{theorem}
\label{thm.ign}
Each mixed equilibrium of the Gangster game has the mixed strategy of each player equal to ${\mathcal R}_1$.
\end{theorem}
\begin{proof} 
We first show that ${\mathcal R}_1$ played at all positions of \agentset is a mixed equilibrium. Hence let $n$ be a position and let all positions of \agentset different from $n$ follow ${\mathcal R}_1$. We distinguish two cases:

1. $\alpha(p,n,k)Q> F$. If position $n$ follows ${\mathcal R}_1$ then its expected payoff is $-(1-p)F- pQ\alpha(p,n,k)$. If position $n$ violates ${\mathcal R}_1$ then it pays $F$ with probability $(1-p')$ for $p'> p$ and its expected payoff is $-(1-p')F- p'Q\alpha(p,n,k)$ and thus it will decrease.

2.  Expected payoff of the critical position $n_1$ following ${\mathcal R}_1$ is equal to $-Q\alpha(p,n_1,k)$. If $n_1$ does not follow ${\mathcal R}_1$ then it pays $F$ with some probability $0< 1-p'$ for $p'\geq p$ and thus its expected payoff will decrease to $-(1-p')F- p'Q\alpha(p,n_1,k)$.

3. For $n> n_1$, the expected payoff is bigger than $-\alpha(p,n_1,k)Q$ so the same argument applies.

\begin{remark}
Note that since $n_1,\ldots,n_1+k-1$ all pay zero according to ${\mathcal R}_1$, the expected payoff for the subsequent positions is $0$.
\end{remark}

Further, by contradiction we easily observe that the mixed equilibrium is unique. If there is another one, then we consider the first player $a$ in \agentset whose mixed strategy deviates from ${\mathcal R}_1$, and we observe that fixing the strategies of the remaining players and changing the strategy of $a$ to ${\mathcal R}_1$ gives $a$ a bigger payoff.

\end{proof}



This observation, interpreted for the traffic fines collection says that a publicity campaign which decreases the probability of ignorance virtually increases the number of state employees assigned to processing the fines collection. 

\begin{theorem}
\label{thm.avef}
Let $\mathbb R$ be the set of Gangster games where all the players follow strategy $\mathcal{R}_1$. Then $\mathbb R$ exhibits the avalanche effect.
\end{theorem}
\begin{proof}
Let $(R^i)$ be an infinite sequence of Gangster games such that $I_{R^i}\setminus \{p(R^i)\}$\todo{D: This is not the input anymore.} is constant and $p(R^i)$ goes to zero. It follows from Theorem \ref{thm.p} that for each $\epsilon>0$ there is $i(\epsilon)$ so that for each $i> i(\epsilon)$, the expectation of each individual payoff of $R^i$ is at most $-F+\epsilon$. This proves the theorem.
\end{proof}

As a final remark, the Gangster game when partial payments are allowed, i.e., $Q>F>1$ is much harder to analyze by analytic methods. \todo{experiments?}


\subsection{The 2-Fines Game}
\label{sub.ex}
The most practical variant of \gamename for collecting traffic fines has parameters $Q>F=1$, $T=w$ and $x= 0$ and thus we call it {\em w-Fines game}. The Gangster game is thus the 1-Fines game.

In this part, we describe the solution of 2-Fines game.


 \begin{definition}
 \label{def.exppp}
For $m<n-k$, we let $\mathcal G_1^m(p,n,k)$ be the expectation of the payoff at position $n(m)$ of the Gangster game when all the players follow ${\mathcal R}_1$, where $n(m)$ is the random variable obtained from $n-k$ by $m$ independent events, each event consisting of subtracting $1$ with probability $1-p$. Hence, the expectation of $n(m)$ is $pm+n-k-m$.
\end{definition}

Next definition is important and quite recursive. For $n=1, \ldots$ we define inductively functions $m(p,n,k)$, $c_2(p,n,k)$, strategy ${\mathcal R}_2$ and critical position $n_2$. 
%The meaning of $m(p,n,k)$ is the expected number of positions smaller than $n$ which pay zero following strategy ${\mathcal D}_2$ in the first round. 

\begin{definition}
\label{def.2df}
For $n=k+1, \ldots$ we define inductively functions $m= m(p,n,k)$, $c_2(p,n,k)$, strategy ${\mathcal R}_2$ and critical position $r_2$ as follows.
\begin{itemize}
    \item $m(p,k+1,k)= 0$,
    \item 
    $
    c_2(p,n,k)= c_1(p,n,k)+ (1-\alpha'(p,n,k))\mathcal G_1^m(p,n,k),
    $
    \item
    If $c_2(p,n-1,k)> F$ then let $m= m(p,n,k)= n-k-1$,
    \item
    If $c_2(p,n-1,k)\leq F$ then let $r_2$ be smallest such that $c_2(p,r_2,k)\leq F$,
    \item
    If $c_2(p,n-1,k)\leq F$ then $m(p,n,k)= r_2-k-1$,
    \item
    the mixed strategy ${\mathcal R}_2$ for a player $a$ is: in the first round, pay $F$ with probability $1-p$ if $c_2(p,n_a,k)> F$ and pay $0$ otherwise. In the second round, follow mixed strategy ${\mathcal R}_1$.
    \end{itemize}
\end{definition}
\begin{lemma}
\label{l.comp}
$r_1+k\leq r_2.$
\end{lemma}
\begin{proof}
We first note that by definition, $m(p,r_2,k)= (r_2-k-1)$.

Abusing notation, $r_2$ is smallest such that $$c_1(r_2)+ (1-\alpha'(r_2))\mathcal G_1^{r_2-k-1}(r_2)\leq F.$$

If $r_2< r_1+k$ then $\mathcal G_1^{r_2-k-1}(r_2)> F$ by the definition of $r_1$, contradicting the defining inequality for $r_2$.

\end{proof}
\begin{proposition}
\label{p.aaa}
If $Q>>F$ then $r_1(2k)< 2r_1(k)$.
\end{proposition}
\begin{proof}
It suffices to show that $\alpha(p,r_1,k)\geq \alpha(p,2r_1,2k)$. If $r_1p \leq k$ then $\alpha(p,r_1,k)> F/Q$ contradicting the definition of $r_1$ and thus $r_1p > k$ and the statement follows from Proposition \ref{p.aa}.

\end{proof}


\begin{theorem}
\label{thm.p2}
Let $r_2$ be the critical position and let all players follow ${\mathcal R}_2$ in the 2-Fines game. The expected payoff $G_2(p,r_2,k)$ of player $a$ is: (1) If $n_a< r_2$ then $G_2(p,n_a,k)= (1-p)F+ pc_2(p,n_a,k)$, (2) If $r_2\geq n_a$ then $G_2(p,n_a,k)= c_2(p,n_a,k)$. 
%and (3) $G_2(p,r_2,K)= G_1(p,m(p,n,K)+1,K)$ when $r_2\geq n_2+K$. 
The total expected payoff, denoted by $T_2(p,x_0,k)$ is
$
T_2(p,x_0,k)= (1-p)F(r_1+r_2-k-2) + 2Qk
$.
\end{theorem}


\begin{theorem}
\label{thm.ign}
The strategy of each player in each mixed equilibrium of the 2-Fines game is ${\mathcal R}_2$. Moreover, if $\mathbb F$ denotes the set of 2-Fines games where all players follow ${\mathcal R}_2$, then $\mathbb F$ exhibits the avalanche effect.
\end{theorem}
\begin{proof} 
The second statement follows from Theorem \ref{thm.p2}. We now show that ${\mathcal R}_2$ played at all positions of \agentset is a mixed equilibrium. Hence let $n$ be a position and let all positions of \agentset different from $n$ follow ${\mathcal R}_2$. We distinguish two cases:

1. $c_2(p,n,k)> F$. If position $n$ follows ${\mathcal R}_2$ then its expected payoff is $-(1-p)F- pc_2(p,n,k)$. If position $n$ violates ${\mathcal D}_2$ then it pays $F$ with probability $(1-p')$ for $p'> p$ and its expected payoff is $-(1-p')F- p'c_2(p,n,k)$ and thus it will decrease.

2.  Expected payoff of the critical position $r_2$ following ${\mathcal R}_2$ is equal to $-c_2(p,r_2,k)$. If $r_2$ does not follow ${\mathcal R}_2$ then it pays $F$ with some probability $0< 1-p'$ for $p'\geq p$ and thus its expected payoff will decrease to $-(1-p')F- p'Q\alpha(p,r_2,k)$.

3. For $n> r_2$, the expected payoff is bigger than $-c_2(p,r_2,k)$ so the same argument applies.

Finally, the uniqueness is proved as in the proof of Theorem \ref{thm.ign}.

\end{proof}
In $w$-Fines game, $k$ administrators settle fines
in $w$ rounds. Hence, they effectively need to perform $kw$ tasks. A natural question and ourwork in progress is, if we fix the number of tasks, what is the setting of $w$ and $k$ for maximising the total payoff? We report a very interesting partial answer to this basic question below. 
\begin{corollary}
\label{c.2fines}
If $Q>>F$ then the equilibrium strategy for $w=2, k$ give better total payoff than the equilibrium strategy for $w=1, 2k$.
\end{corollary}
\begin{proof}
This follows from Theorem \ref{thm.p}, Theorem \ref{thm.p2} and Proposition \ref{p.aaa}.
\end{proof}







